The California Legacy Survey IV. Lonely, Poor, and Eccentric: A Comparison Between Solitary and Neighborly Gas Giants

We compare systems with single giant planets to systems with multiple giant planets using a catalog of planets from a high-precision radial velocity survey of FGKM stars. Our comparison focuses on orbital properties, planet masses, and host star properties. We use hierarchical methods to model the orbital eccentricity distributions of giant singles and giant multis, and find that the distributions are distinct. The multiple giant planets typically have moderate eccentricities and their eccentricity distribution extends to $e=0.47$ (90th percentile), while the single giant planets have a pile-up of nearly circular orbits and a long tail that extends to $e=0.77$. We determine that stellar hosts of multiple giants are distinctly more metal-rich than hosts of solitary giants, with respective mean metallicities $0.228\pm0.027$ vs. $0.129\pm0.019$ dex. We measure the distinct occurrence distributions of single and multiple giants with respect to orbital separation, and find that single gas giants have a $\sim$2.3$\sigma$ significant hot ($a<0.06$) Jupiter pile-up not seen among multi giant systems. We find that the median mass ($\msini$ ) of giants in multiples is nearly double that of single giants (1.71 $\mjup$ vs. 0.92 $\mjup$ ). We find that giant planets in the same system have correlated masses, analogous to the `peas in a pod' effect seen among less massive planets.

==> system_macros.tex <==
\newcommand{\ddigTEFF}{\ensuremath{5261 \pm 100}\xspace} 
 \newcommand{\hieeTEFF}{\ensuremath{6379 \pm 100}\xspace} 
 \newcommand{\hbagTEFF}{\ensuremath{5607 \pm 100}\xspace} 
 \newcommand{\jjhiTEFF}{\ensuremath{5961 \pm 100}\xspace} 
 \newcommand{\fcabTEFF}{\ensuremath{6019 \pm 100}\xspace} 
 \newcommand{\eidfTEFF}{\ensuremath{5839 \pm 100}\xspace} 
 \newcommand{\hehhTEFF}{\ensuremath{5705 \pm 100}\xspace} 
 \newcommand{\jifiTEFF}{\ensuremath{4217 \pm 70}\xspace} 
 \newcommand{\iahiTEFF}{\ensuremath{5478 \pm 100}\xspace} 
 \newcommand{\aiggTEFF}{\ensuremath{6044 \pm 100}\xspace} 
 \newcommand{\jgjjTEFF}{\ensuremath{5340 \pm 100}\xspace} 
 \newcommand{\hhedTEFF}{\ensuremath{4915 \pm 100}\xspace} 
 \newcommand{\befbTEFF}{\ensuremath{5163 \pm 100}\xspace} 
 \newcommand{\jgfhTEFF}{\ensuremath{6132 \pm 100}\xspace} 
 \newcommand{\eaccTEFF}{\ensuremath{5832 \pm 100}\xspace} 
 \newcommand{\dcijTEFF}{\ensuremath{6053 \pm 100}\xspace} 
 \newcommand{\bejgTEFF}{\ensuremath{5435 \pm 100}\xspace} 
 \newcommand{\bajiTEFF}{\ensuremath{5625 \pm 100}\xspace} 
 \newcommand{\bcgdTEFF}{\ensuremath{5679 \pm 100}\xspace} 
 \newcommand{\fffdTEFF}{\ensuremath{5867 \pm 100}\xspace} 
 \newcommand{\ecdcTEFF}{\ensuremath{4271 \pm 70}\xspace} 
 \newcommand{\dcbjTEFF}{\ensuremath{5865 \pm 100}\xspace} 
 \newcommand{\ddeiTEFF}{\ensuremath{4836 \pm 100}\xspace} 
 \newcommand{\fdijTEFF}{\ensuremath{5373 \pm 100}\xspace} 
 \newcommand{\gafeTEFF}{\ensuremath{5875 \pm 100}\xspace} 
 \newcommand{\bhiiTEFF}{\ensuremath{5612 \pm 100}\xspace} 
 \newcommand{\bbggTEFF}{\ensuremath{4868 \pm 100}\xspace} 
 \newcommand{\dbfaTEFF}{\ensuremath{5476 \pm 100}\xspace} 
 \newcommand{\ccdhTEFF}{\ensuremath{5853 \pm 100}\xspace} 
 \newcommand{\eicdTEFF}{\ensuremath{5496 \pm 100}\xspace} 
 \newcommand{\bggeTEFF}{\ensuremath{6103 \pm 100}\xspace} 
 \newcommand{\gcidTEFF}{\ensuremath{5685 \pm 100}\xspace} 
 \newcommand{\jfjgTEFF}{\ensuremath{4507 \pm 110}\xspace} 
 \newcommand{\baeiTEFF}{\ensuremath{5773 \pm 100}\xspace} 
 \newcommand{\bjieTEFF}{\ensuremath{5274 \pm 100}\xspace} 
 \newcommand{\gghbTEFF}{\ensuremath{5474 \pm 100}\xspace} 
 \newcommand{\ggacTEFF}{\ensuremath{4455 \pm 70}\xspace} 
 \newcommand{\egijTEFF}{\ensuremath{5442 \pm 100}\xspace} 
 \newcommand{\hadfTEFF}{\ensuremath{5533 \pm 100}\xspace} 
 \newcommand{\hidfTEFF}{\ensuremath{5942 \pm 100}\xspace} 
 \newcommand{\bebbTEFF}{\ensuremath{4495 \pm 70}\xspace} 
 \newcommand{\ecdiTEFF}{\ensuremath{5741 \pm 100}\xspace} 
 \newcommand{\gedgTEFF}{\ensuremath{5352 \pm 100}\xspace} 
 \newcommand{\jgbhTEFF}{\ensuremath{5166 \pm 100}\xspace} 
 \newcommand{\ghijTEFF}{\ensuremath{5246 \pm 100}\xspace} 
 \newcommand{\fdecTEFF}{\ensuremath{5528 \pm 100}\xspace} 
 \newcommand{\deffTEFF}{\ensuremath{5310 \pm 100}\xspace} 
 \newcommand{\hbdaTEFF}{\ensuremath{4237 \pm 70}\xspace} 
 \newcommand{\eiadTEFF}{\ensuremath{5748 \pm 100}\xspace} 
 \newcommand{\ifgjTEFF}{\ensuremath{4526 \pm 110}\xspace} 
 \newcommand{\cffcTEFF}{\ensuremath{3449 \pm 70}\xspace} 
 \newcommand{\ddigLOGG}{\ensuremath{4.470 \pm 0.080}\xspace} 
 \newcommand{\hieeLOGG}{\ensuremath{4.230 \pm 0.080}\xspace} 
 \newcommand{\hbagLOGG}{\ensuremath{4.010 \pm 0.080}\xspace} 
 \newcommand{\jjhiLOGG}{\ensuremath{4.330 \pm 0.080}\xspace} 
 \newcommand{\fcabLOGG}{\ensuremath{4.180 \pm 0.080}\xspace} 
 \newcommand{\eidfLOGG}{\ensuremath{4.420 \pm 0.080}\xspace} 
 \newcommand{\hehhLOGG}{\ensuremath{4.450 \pm 0.080}\xspace} 
 \newcommand{\jifiLOGG}{\ensuremath{4.62 \pm 0.20}\xspace} 
 \newcommand{\iahiLOGG}{\ensuremath{4.020 \pm 0.080}\xspace} 
 \newcommand{\aiggLOGG}{\ensuremath{4.400 \pm 0.080}\xspace} 
 \newcommand{\jgjjLOGG}{\ensuremath{4.450 \pm 0.083}\xspace} 
 \newcommand{\hhedLOGG}{\ensuremath{3.580 \pm 0.080}\xspace} 
 \newcommand{\befbLOGG}{\ensuremath{4.530 \pm 0.080}\xspace} 
 \newcommand{\jgfhLOGG}{\ensuremath{4.130 \pm 0.080}\xspace} 
 \newcommand{\eaccLOGG}{\ensuremath{4.430 \pm 0.080}\xspace} 
 \newcommand{\dcijLOGG}{\ensuremath{3.900 \pm 0.080}\xspace} 
 \newcommand{\bejgLOGG}{\ensuremath{4.470 \pm 0.080}\xspace} 
 \newcommand{\bajiLOGG}{\ensuremath{4.290 \pm 0.083}\xspace} 
 \newcommand{\bcgdLOGG}{\ensuremath{4.320 \pm 0.083}\xspace} 
 \newcommand{\fffdLOGG}{\ensuremath{4.390 \pm 0.081}\xspace} 
 \newcommand{\ecdcLOGG}{\ensuremath{4.60 \pm 0.20}\xspace} 
 \newcommand{\dcbjLOGG}{\ensuremath{3.990 \pm 0.080}\xspace} 
 \newcommand{\ddeiLOGG}{\ensuremath{4.550 \pm 0.084}\xspace} 
 \newcommand{\fdijLOGG}{\ensuremath{4.450 \pm 0.085}\xspace} 
 \newcommand{\gafeLOGG}{\ensuremath{4.280 \pm 0.081}\xspace} 
 \newcommand{\bhiiLOGG}{\ensuremath{4.450 \pm 0.080}\xspace} 
 \newcommand{\bbggLOGG}{\ensuremath{4.530 \pm 0.080}\xspace} 
 \newcommand{\dbfaLOGG}{\ensuremath{4.270 \pm 0.080}\xspace} 
 \newcommand{\ccdhLOGG}{\ensuremath{4.180 \pm 0.081}\xspace} 
 \newcommand{\eicdLOGG}{\ensuremath{4.420 \pm 0.080}\xspace} 
 \newcommand{\bggeLOGG}{\ensuremath{4.120 \pm 0.081}\xspace} 
 \newcommand{\gcidLOGG}{\ensuremath{4.23 \pm 0.10}\xspace} 
 \newcommand{\jfjgLOGG}{\ensuremath{4.61 \pm 0.20}\xspace} 
 \newcommand{\baeiLOGG}{\ensuremath{4.31 \pm 0.10}\xspace} 
 \newcommand{\bjieLOGG}{\ensuremath{4.490 \pm 0.083}\xspace} 
 \newcommand{\gghbLOGG}{\ensuremath{3.990 \pm 0.081}\xspace} 
 \newcommand{\ggacLOGG}{\ensuremath{4.57 \pm 0.20}\xspace} 
 \newcommand{\egijLOGG}{\ensuremath{4.510 \pm 0.085}\xspace} 
 \newcommand{\hadfLOGG}{\ensuremath{4.470 \pm 0.085}\xspace} 
 \newcommand{\hidfLOGG}{\ensuremath{4.580 \pm 0.081}\xspace} 
 \newcommand{\bebbLOGG}{\ensuremath{4.60 \pm 0.20}\xspace} 
 \newcommand{\ecdiLOGG}{\ensuremath{4.14 \pm 0.10}\xspace} 
 \newcommand{\gedgLOGG}{\ensuremath{4.530 \pm 0.083}\xspace} 
 \newcommand{\jgbhLOGG}{\ensuremath{4.630 \pm 0.081}\xspace} 
 \newcommand{\ghijLOGG}{\ensuremath{4.480 \pm 0.081}\xspace} 
 \newcommand{\fdecLOGG}{\ensuremath{4.350 \pm 0.085}\xspace} 
 \newcommand{\deffLOGG}{\ensuremath{4.420 \pm 0.081}\xspace} 
 \newcommand{\hbdaLOGG}{\ensuremath{4.55 \pm 0.20}\xspace} 
 \newcommand{\eiadLOGG}{\ensuremath{4.380 \pm 0.085}\xspace} 
 \newcommand{\ifgjLOGG}{\ensuremath{4.63 \pm 0.20}\xspace} 
 \newcommand{\cffcLOGG}{\ensuremath{4.60 \pm 0.20}\xspace} 
 \newcommand{\ddigFEH}{\ensuremath{0.040 \pm 0.043}\xspace} 
 \newcommand{\hieeFEH}{\ensuremath{-0.060 \pm 0.044}\xspace} 
 \newcommand{\hbagFEH}{\ensuremath{0.470 \pm 0.044}\xspace} 
 \newcommand{\jjhiFEH}{\ensuremath{-0.250 \pm 0.044}\xspace} 
 \newcommand{\fcabFEH}{\ensuremath{0.140 \pm 0.044}\xspace} 
 \newcommand{\eidfFEH}{\ensuremath{-0.110 \pm 0.044}\xspace} 
 \newcommand{\hehhFEH}{\ensuremath{0.050 \pm 0.044}\xspace} 
 \newcommand{\jifiFEH}{\ensuremath{-0.28 \pm 0.12}\xspace} 
 \newcommand{\iahiFEH}{\ensuremath{0.350 \pm 0.043}\xspace} 
 \newcommand{\aiggFEH}{\ensuremath{0.300 \pm 0.044}\xspace} 
 \newcommand{\jgjjFEH}{\ensuremath{0.180 \pm 0.046}\xspace} 
 \newcommand{\hhedFEH}{\ensuremath{0.430 \pm 0.043}\xspace} 
 \newcommand{\befbFEH}{\ensuremath{0.040 \pm 0.043}\xspace} 
 \newcommand{\jgfhFEH}{\ensuremath{-0.140 \pm 0.044}\xspace} 
 \newcommand{\eaccFEH}{\ensuremath{-0.440 \pm 0.044}\xspace} 
 \newcommand{\dcijFEH}{\ensuremath{0.240 \pm 0.044}\xspace} 
 \newcommand{\bejgFEH}{\ensuremath{0.050 \pm 0.043}\xspace} 
 \newcommand{\bajiFEH}{\ensuremath{0.340 \pm 0.046}\xspace} 
 \newcommand{\bcgdFEH}{\ensuremath{0.230 \pm 0.046}\xspace} 
 \newcommand{\fffdFEH}{\ensuremath{0.040 \pm 0.044}\xspace} 
 \newcommand{\ecdcFEH}{\ensuremath{0.03 \pm 0.12}\xspace} 
 \newcommand{\dcbjFEH}{\ensuremath{-0.050 \pm 0.044}\xspace} 
 \newcommand{\ddeiFEH}{\ensuremath{0.000 \pm 0.046}\xspace} 
 \newcommand{\fdijFEH}{\ensuremath{0.220 \pm 0.047}\xspace} 
 \newcommand{\gafeFEH}{\ensuremath{0.040 \pm 0.044}\xspace} 
 \newcommand{\bhiiFEH}{\ensuremath{-0.050 \pm 0.044}\xspace} 
 \newcommand{\bbggFEH}{\ensuremath{-0.270 \pm 0.044}\xspace} 
 \newcommand{\dbfaFEH}{\ensuremath{0.370 \pm 0.044}\xspace} 
 \newcommand{\ccdhFEH}{\ensuremath{-0.000 \pm 0.044}\xspace} 
 \newcommand{\eicdFEH}{\ensuremath{0.060 \pm 0.044}\xspace} 
 \newcommand{\bggeFEH}{\ensuremath{-0.060 \pm 0.044}\xspace} 
 \newcommand{\gcidFEH}{\ensuremath{-0.135 \pm 0.060}\xspace} 
 \newcommand{\jfjgFEH}{\ensuremath{-0.040 \pm 0.080}\xspace} 
 \newcommand{\baeiFEH}{\ensuremath{0.038 \pm 0.060}\xspace} 
 \newcommand{\bjieFEH}{\ensuremath{-0.030 \pm 0.046}\xspace} 
 \newcommand{\gghbFEH}{\ensuremath{0.330 \pm 0.044}\xspace} 
 \newcommand{\ggacFEH}{\ensuremath{-0.10 \pm 0.12}\xspace} 
 \newcommand{\egijFEH}{\ensuremath{-0.100 \pm 0.047}\xspace} 
 \newcommand{\hadfFEH}{\ensuremath{-0.070 \pm 0.047}\xspace} 
 \newcommand{\hidfFEH}{\ensuremath{-0.450 \pm 0.045}\xspace} 
 \newcommand{\bebbFEH}{\ensuremath{0.08 \pm 0.12}\xspace} 
 \newcommand{\ecdiFEH}{\ensuremath{0.353 \pm 0.060}\xspace} 
 \newcommand{\gedgFEH}{\ensuremath{-0.080 \pm 0.046}\xspace} 
 \newcommand{\jgbhFEH}{\ensuremath{-0.710 \pm 0.045}\xspace} 
 \newcommand{\ghijFEH}{\ensuremath{0.120 \pm 0.045}\xspace} 
 \newcommand{\fdecFEH}{\ensuremath{0.180 \pm 0.047}\xspace} 
 \newcommand{\deffFEH}{\ensuremath{0.240 \pm 0.045}\xspace} 
 \newcommand{\hbdaFEH}{\ensuremath{0.13 \pm 0.12}\xspace} 
 \newcommand{\eiadFEH}{\ensuremath{0.030 \pm 0.048}\xspace} 
 \newcommand{\ifgjFEH}{\ensuremath{0.040 \pm 0.080}\xspace} 
 \newcommand{\cffcFEH}{\ensuremath{0.00 \pm 0.12}\xspace} 
 \newcommand{\ddigSVAL}{0.1463\xspace} 
 \newcommand{\hieeSVAL}{0.136\xspace} 
 \newcommand{\hbagSVAL}{0.1361\xspace} 
 \newcommand{\jjhiSVAL}{0.1407\xspace} 
 \newcommand{\fcabSVAL}{0.1337\xspace} 
 \newcommand{\eidfSVAL}{0.1616\xspace} 
 \newcommand{\hehhSVAL}{0.186\xspace} 
 \newcommand{\jifiSVAL}{0.4492\xspace} 
 \newcommand{\iahiSVAL}{0.1382\xspace} 
 \newcommand{\aiggSVAL}{0.2772\xspace} 
 \newcommand{\jgjjSVAL}{0.2936\xspace} 
 \newcommand{\hhedSVAL}{0.173\xspace} 
 \newcommand{\befbSVAL}{0.3516\xspace} 
 \newcommand{\jgfhSVAL}{0.1181\xspace} 
 \newcommand{\eaccSVAL}{0.1411\xspace} 
 \newcommand{\dcijSVAL}{0.119\xspace} 
 \newcommand{\bejgSVAL}{0.196\xspace} 
 \newcommand{\bajiSVAL}{0.1281\xspace} 
 \newcommand{\bcgdSVAL}{0.1435\xspace} 
 \newcommand{\fffdSVAL}{0.1586\xspace} 
 \newcommand{\ecdcSVAL}{1.018\xspace} 
 \newcommand{\dcbjSVAL}{0.1276\xspace} 
 \newcommand{\ddeiSVAL}{0.4628\xspace} 
 \newcommand{\fdijSVAL}{0.2097\xspace} 
 \newcommand{\gafeSVAL}{0.1432\xspace} 
 \newcommand{\bhiiSVAL}{0.1391\xspace} 
 \newcommand{\bbggSVAL}{0.1761\xspace} 
 \newcommand{\dbfaSVAL}{0.1325\xspace} 
 \newcommand{\ccdhSVAL}{0.1414\xspace} 
 \newcommand{\eicdSVAL}{0.1419\xspace} 
 \newcommand{\bggeSVAL}{0.1335\xspace} 
 \newcommand{\gcidSVAL}{0.1761\xspace} 
 \newcommand{\jfjgSVAL}{0.4743\xspace} 
 \newcommand{\baeiSVAL}{0.1432\xspace} 
 \newcommand{\bjieSVAL}{0.1567\xspace} 
 \newcommand{\gghbSVAL}{0.1211\xspace} 
 \newcommand{\ggacSVAL}{0.2961\xspace} 
 \newcommand{\egijSVAL}{0.1663\xspace} 
 \newcommand{\hadfSVAL}{0.1481\xspace} 
 \newcommand{\hidfSVAL}{0.1387\xspace} 
 \newcommand{\bebbSVAL}{0.612\xspace} 
 \newcommand{\ecdiSVAL}{0.127\xspace} 
 \newcommand{\gedgSVAL}{0.1787\xspace} 
 \newcommand{\jgbhSVAL}{0.2003\xspace} 
 \newcommand{\ghijSVAL}{0.1627\xspace} 
 \newcommand{\fdecSVAL}{0.183\xspace} 
 \newcommand{\deffSVAL}{0.1538\xspace} 
 \newcommand{\hbdaSVAL}{0.7891\xspace} 
 \newcommand{\eiadSVAL}{0.1433\xspace} 
 \newcommand{\ifgjSVAL}{0.728\xspace} 
 \newcommand{\cffcSVAL}{0.5806\xspace} 
 \newcommand{\ddigRPHK}{$-$5.114\xspace} 
 \newcommand{\hieeRPHK}{$-$5.147\xspace} 
 \newcommand{\hbagRPHK}{$-$5.179\xspace} 
 \newcommand{\jjhiRPHK}{$-$5.128\xspace} 
 \newcommand{\fcabRPHK}{$-$5.193\xspace} 
 \newcommand{\eidfRPHK}{$-$4.984\xspace} 
 \newcommand{\hehhRPHK}{$-$4.875\xspace} 
 \newcommand{\jifiRPHK}{$-$4.905\xspace} 
 \newcommand{\iahiRPHK}{$-$5.16\xspace} 
 \newcommand{\aiggRPHK}{$-$4.526\xspace} 
 \newcommand{\jgjjRPHK}{$-$4.647\xspace} 
 \newcommand{\hhedRPHK}{$-$5.06\xspace} 
 \newcommand{\befbRPHK}{$-$4.603\xspace} 
 \newcommand{\jgfhRPHK}{$-$5.407\xspace} 
 \newcommand{\eaccRPHK}{$-$5.133\xspace} 
 \newcommand{\dcijRPHK}{$-$5.393\xspace} 
 \newcommand{\bejgRPHK}{$-$4.878\xspace} 
 \newcommand{\bajiRPHK}{$-$5.253\xspace} 
 \newcommand{\bcgdRPHK}{$-$5.12\xspace} 
 \newcommand{\fffdRPHK}{$-$4.999\xspace} 
 \newcommand{\ecdcRPHK}{$-$4.519\xspace} 
 \newcommand{\dcbjRPHK}{$-$5.267\xspace} 
 \newcommand{\ddeiRPHK}{$-$4.594\xspace} 
 \newcommand{\fdijRPHK}{$-$4.843\xspace} 
 \newcommand{\gafeRPHK}{$-$5.112\xspace} 
 \newcommand{\bhiiRPHK}{$-$5.155\xspace} 
 \newcommand{\bbggRPHK}{$-$5.063\xspace} 
 \newcommand{\dbfaRPHK}{$-$5.201\xspace} 
 \newcommand{\ccdhRPHK}{$-$5.129\xspace} 
 \newcommand{\eicdRPHK}{$-$5.135\xspace} 
 \newcommand{\bggeRPHK}{$-$5.189\xspace} 
 \newcommand{\gcidRPHK}{$-$4.923\xspace} 
 \newcommand{\jfjgRPHK}{$-$4.735\xspace} 
 \newcommand{\baeiRPHK}{$-$5.119\xspace} 
 \newcommand{\bjieRPHK}{$-$5.061\xspace} 
 \newcommand{\gghbRPHK}{$-$5.304\xspace} 
 \newcommand{\ggacRPHK}{$-$4.972\xspace} 
 \newcommand{\egijRPHK}{$-$4.999\xspace} 
 \newcommand{\hadfRPHK}{$-$5.093\xspace} 
 \newcommand{\hidfRPHK}{$-$5.148\xspace} 
 \newcommand{\bebbRPHK}{$-$4.627\xspace} 
 \newcommand{\ecdiRPHK}{$-$5.273\xspace} 
 \newcommand{\gedgRPHK}{$-$4.957\xspace} 
 \newcommand{\jgbhRPHK}{$-$4.916\xspace} 
 \newcommand{\ghijRPHK}{$-$5.037\xspace} 
 \newcommand{\fdecRPHK}{$-$4.914\xspace} 
 \newcommand{\deffRPHK}{$-$5.073\xspace} 
 \newcommand{\hbdaRPHK}{$-$4.648\xspace} 
 \newcommand{\eiadRPHK}{$-$5.119\xspace} 
 \newcommand{\ifgjRPHK}{$-$4.534\xspace} 
 \newcommand{\cffcRPHK}{$-$5.183\xspace} 
 \newcommand{\ddigVSINI}{\ensuremath{1.1 \pm 1.0}\xspace} 
 \newcommand{\hieeVSINI}{\ensuremath{12.3 \pm 1.0}\xspace} 
 \newcommand{\hbagVSINI}{\ensuremath{3.0 \pm 1.0}\xspace} 
 \newcommand{\jjhiVSINI}{\ensuremath{1.6 \pm 1.0}\xspace} 
 \newcommand{\fcabVSINI}{\ensuremath{0.1 \pm 1.0}\xspace} 
 \newcommand{\eidfVSINI}{\ensuremath{1.6 \pm 1.0}\xspace} 
 \newcommand{\hehhVSINI}{\ensuremath{2.3 \pm 1.0}\xspace} 
 \newcommand{\jifiVSINI}{---\xspace} 
 \newcommand{\iahiVSINI}{\ensuremath{3.0 \pm 1.0}\xspace} 
 \newcommand{\aiggVSINI}{\ensuremath{13.3 \pm 1.0}\xspace} 
 \newcommand{\jgjjVSINI}{\ensuremath{2.8 \pm 1.0}\xspace} 
 \newcommand{\hhedVSINI}{\ensuremath{0.1 \pm 1.0}\xspace} 
 \newcommand{\befbVSINI}{\ensuremath{2.6 \pm 1.0}\xspace} 
 \newcommand{\jgfhVSINI}{\ensuremath{0.9 \pm 1.0}\xspace} 
 \newcommand{\eaccVSINI}{\ensuremath{0.1 \pm 1.0}\xspace} 
 \newcommand{\dcijVSINI}{\ensuremath{9.4 \pm 1.0}\xspace} 
 \newcommand{\bejgVSINI}{\ensuremath{1.8 \pm 1.0}\xspace} 
 \newcommand{\bajiVSINI}{\ensuremath{2.2 \pm 1.0}\xspace} 
 \newcommand{\bcgdVSINI}{\ensuremath{1.5 \pm 1.0}\xspace} 
 \newcommand{\fffdVSINI}{\ensuremath{2.0 \pm 1.0}\xspace} 
 \newcommand{\ecdcVSINI}{---\xspace} 
 \newcommand{\dcbjVSINI}{\ensuremath{4.0 \pm 1.0}\xspace} 
 \newcommand{\ddeiVSINI}{\ensuremath{2.7 \pm 1.0}\xspace} 
 \newcommand{\fdijVSINI}{\ensuremath{2.7 \pm 1.0}\xspace} 
 \newcommand{\gafeVSINI}{\ensuremath{1.9 \pm 1.0}\xspace} 
 \newcommand{\bhiiVSINI}{\ensuremath{1.1 \pm 1.0}\xspace} 
 \newcommand{\bbggVSINI}{\ensuremath{0.1 \pm 1.0}\xspace} 
 \newcommand{\dbfaVSINI}{\ensuremath{2.2 \pm 1.0}\xspace} 
 \newcommand{\ccdhVSINI}{\ensuremath{1.9 \pm 1.0}\xspace} 
 \newcommand{\eicdVSINI}{\ensuremath{1.7 \pm 1.0}\xspace} 
 \newcommand{\bggeVSINI}{\ensuremath{5.6 \pm 1.0}\xspace} 
 \newcommand{\gcidVSINI}{\ensuremath{0.1 \pm 1.0}\xspace} 
 \newcommand{\jfjgVSINI}{---\xspace} 
 \newcommand{\baeiVSINI}{\ensuremath{1.8 \pm 1.0}\xspace} 
 \newcommand{\bjieVSINI}{\ensuremath{0.7 \pm 1.0}\xspace} 
 \newcommand{\gghbVSINI}{\ensuremath{2.9 \pm 1.0}\xspace} 
 \newcommand{\ggacVSINI}{---\xspace} 
 \newcommand{\egijVSINI}{\ensuremath{1.9 \pm 1.0}\xspace} 
 \newcommand{\hadfVSINI}{\ensuremath{1.5 \pm 1.0}\xspace} 
 \newcommand{\hidfVSINI}{\ensuremath{0.1 \pm 1.0}\xspace} 
 \newcommand{\bebbVSINI}{---\xspace} 
 \newcommand{\ecdiVSINI}{\ensuremath{2.5 \pm 1.0}\xspace} 
 \newcommand{\gedgVSINI}{\ensuremath{1.3 \pm 1.0}\xspace} 
 \newcommand{\jgbhVSINI}{\ensuremath{0.1 \pm 1.0}\xspace} 
 \newcommand{\ghijVSINI}{\ensuremath{1.6 \pm 1.0}\xspace} 
 \newcommand{\fdecVSINI}{\ensuremath{2.1 \pm 1.0}\xspace} 
 \newcommand{\deffVSINI}{\ensuremath{1.9 \pm 1.0}\xspace} 
 \newcommand{\hbdaVSINI}{---\xspace} 
 \newcommand{\eiadVSINI}{\ensuremath{1.6 \pm 1.0}\xspace} 
 \newcommand{\ifgjVSINI}{---\xspace} 
 \newcommand{\cffcVSINI}{---\xspace} 
 \newcommand{\ddigMSTAR}{\ensuremath{0.86 \pm 0.03}\xspace} 
 \newcommand{\hieeMSTAR}{\ensuremath{1.18 \pm 0.05}\xspace} 
 \newcommand{\hbagMSTAR}{\ensuremath{1.22 \pm 0.10}\xspace} 
 \newcommand{\jjhiMSTAR}{\ensuremath{0.92 \pm 0.04}\xspace} 
 \newcommand{\fcabMSTAR}{\ensuremath{1.17 \pm 0.07}\xspace} 
 \newcommand{\eidfMSTAR}{\ensuremath{0.95 \pm 0.04}\xspace} 
 \newcommand{\hehhMSTAR}{\ensuremath{0.98 \pm 0.04}\xspace} 
 \newcommand{\jifiMSTAR}{\ensuremath{0.58 \pm 0.03}\xspace} 
 \newcommand{\iahiMSTAR}{\ensuremath{1.09 \pm 0.07}\xspace} 
 \newcommand{\aiggMSTAR}{\ensuremath{1.21 \pm 0.04}\xspace} 
 \newcommand{\jgjjMSTAR}{\ensuremath{0.92 \pm 0.04}\xspace} 
 \newcommand{\hhedMSTAR}{\ensuremath{1.38 \pm 0.16}\xspace} 
 \newcommand{\befbMSTAR}{\ensuremath{0.84 \pm 0.03}\xspace} 
 \newcommand{\jgfhMSTAR}{\ensuremath{1.06^{+0.07}_{-0.05} }\xspace} 
 \newcommand{\eaccMSTAR}{\ensuremath{0.83 \pm 0.03}\xspace} 
 \newcommand{\dcijMSTAR}{\ensuremath{1.48 \pm 0.12}\xspace} 
 \newcommand{\bejgMSTAR}{\ensuremath{0.90 \pm 0.04}\xspace} 
 \newcommand{\bajiMSTAR}{\ensuremath{1.07 \pm 0.05}\xspace} 
 \newcommand{\bcgdMSTAR}{\ensuremath{1.04 \pm 0.05}\xspace} 
 \newcommand{\fffdMSTAR}{\ensuremath{1.02 \pm 0.04}\xspace} 
 \newcommand{\ecdcMSTAR}{\ensuremath{0.66 \pm 0.03}\xspace} 
 \newcommand{\dcbjMSTAR}{\ensuremath{1.06 \pm 0.07}\xspace} 
 \newcommand{\ddeiMSTAR}{\ensuremath{0.76 \pm 0.03}\xspace} 
 \newcommand{\fdijMSTAR}{\ensuremath{0.94 \pm 0.04}\xspace} 
 \newcommand{\gafeMSTAR}{\ensuremath{1.03 \pm 0.05}\xspace} 
 \newcommand{\bhiiMSTAR}{\ensuremath{0.91 \pm 0.04}\xspace} 
 \newcommand{\bbggMSTAR}{\ensuremath{0.70 \pm 0.03}\xspace} 
 \newcommand{\dbfaMSTAR}{\ensuremath{1.01 \pm 0.05}\xspace} 
 \newcommand{\ccdhMSTAR}{\ensuremath{1.01 \pm 0.05}\xspace} 
 \newcommand{\eicdMSTAR}{\ensuremath{0.91 \pm 0.04}\xspace} 
 \newcommand{\bggeMSTAR}{\ensuremath{1.11^{+0.08}_{-0.06} }\xspace} 
 \newcommand{\gcidMSTAR}{\ensuremath{0.89 \pm 0.04}\xspace} 
 \newcommand{\jfjgMSTAR}{\ensuremath{0.69 \pm 0.03}\xspace} 
 \newcommand{\baeiMSTAR}{\ensuremath{0.99 \pm 0.05}\xspace} 
 \newcommand{\bjieMSTAR}{\ensuremath{0.84 \pm 0.03}\xspace} 
 \newcommand{\gghbMSTAR}{\ensuremath{1.10 \pm 0.07}\xspace} 
 \newcommand{\ggacMSTAR}{\ensuremath{0.67 \pm 0.03}\xspace} 
 \newcommand{\egijMSTAR}{\ensuremath{0.85 \pm 0.03}\xspace} 
 \newcommand{\hadfMSTAR}{\ensuremath{0.88 \pm 0.04}\xspace} 
 \newcommand{\hidfMSTAR}{\ensuremath{0.88 \pm 0.03}\xspace} 
 \newcommand{\bebbMSTAR}{\ensuremath{0.72 \pm 0.03}\xspace} 
 \newcommand{\ecdiMSTAR}{\ensuremath{1.17 \pm 0.09}\xspace} 
 \newcommand{\gedgMSTAR}{\ensuremath{0.84 \pm 0.03}\xspace} 
 \newcommand{\jgbhMSTAR}{\ensuremath{0.67 \pm 0.02}\xspace} 
 \newcommand{\ghijMSTAR}{\ensuremath{0.88 \pm 0.03}\xspace} 
 \newcommand{\fdecMSTAR}{\ensuremath{0.96 \pm 0.04}\xspace} 
 \newcommand{\deffMSTAR}{\ensuremath{0.93 \pm 0.04}\xspace} 
 \newcommand{\hbdaMSTAR}{\ensuremath{0.67 \pm 0.03}\xspace} 
 \newcommand{\eiadMSTAR}{\ensuremath{0.97 \pm 0.04}\xspace} 
 \newcommand{\ifgjMSTAR}{\ensuremath{0.71 \pm 0.03}\xspace} 
 \newcommand{\cffcMSTAR}{\ensuremath{0.32 \pm 0.06}\xspace} 
 \newcommand{\ddigRSTAR}{\ensuremath{0.878 \pm 0.034}\xspace} 
 \newcommand{\hieeRSTAR}{\ensuremath{1.273 \pm 0.042}\xspace} 
 \newcommand{\hbagRSTAR}{\ensuremath{1.750 \pm 0.065}\xspace} 
 \newcommand{\jjhiRSTAR}{\ensuremath{1.093 \pm 0.038}\xspace} 
 \newcommand{\fcabRSTAR}{\ensuremath{1.387 \pm 0.049}\xspace} 
 \newcommand{\eidfRSTAR}{\ensuremath{0.998 \pm 0.036}\xspace} 
 \newcommand{\hehhRSTAR}{\ensuremath{0.952 \pm 0.035}\xspace} 
 \newcommand{\jifiRSTAR}{\ensuremath{0.612 \pm 0.021}\xspace} 
 \newcommand{\iahiRSTAR}{\ensuremath{1.679 \pm 0.065}\xspace} 
 \newcommand{\aiggRSTAR}{\ensuremath{1.227 \pm 0.045}\xspace} 
 \newcommand{\jgjjRSTAR}{\ensuremath{1.138 \pm 0.044}\xspace} 
 \newcommand{\hhedRSTAR}{\ensuremath{3.08 \pm 0.14}\xspace} 
 \newcommand{\befbRSTAR}{\ensuremath{0.774 \pm 0.032}\xspace} 
 \newcommand{\jgfhRSTAR}{\ensuremath{1.554 \pm 0.058}\xspace} 
 \newcommand{\eaccRSTAR}{\ensuremath{0.884 \pm 0.063}\xspace} 
 \newcommand{\dcijRSTAR}{\ensuremath{2.66 \pm 0.11}\xspace} 
 \newcommand{\bejgRSTAR}{\ensuremath{0.924 \pm 0.036}\xspace} 
 \newcommand{\bajiRSTAR}{\ensuremath{1.158 \pm 0.043}\xspace} 
 \newcommand{\bcgdRSTAR}{\ensuremath{1.131^{+0.123}_{-0.095} }\xspace} 
 \newcommand{\fffdRSTAR}{\ensuremath{1.058 \pm 0.039}\xspace} 
 \newcommand{\ecdcRSTAR}{\ensuremath{0.671 \pm 0.023}\xspace} 
 \newcommand{\dcbjRSTAR}{\ensuremath{1.79 \pm 0.10}\xspace} 
 \newcommand{\ddeiRSTAR}{\ensuremath{0.717 \pm 0.031}\xspace} 
 \newcommand{\fdijRSTAR}{\ensuremath{0.905 \pm 0.035}\xspace} 
 \newcommand{\gafeRSTAR}{\ensuremath{1.236 \pm 0.047}\xspace} 
 \newcommand{\bhiiRSTAR}{\ensuremath{1.026 \pm 0.040}\xspace} 
 \newcommand{\bbggRSTAR}{\ensuremath{0.710 \pm 0.030}\xspace} 
 \newcommand{\dbfaRSTAR}{\ensuremath{1.144 \pm 0.049}\xspace} 
 \newcommand{\ccdhRSTAR}{\ensuremath{1.247 \pm 0.045}\xspace} 
 \newcommand{\eicdRSTAR}{\ensuremath{0.995 \pm 0.039}\xspace} 
 \newcommand{\bggeRSTAR}{\ensuremath{1.565 \pm 0.065}\xspace} 
 \newcommand{\gcidRSTAR}{\ensuremath{1.154 \pm 0.044}\xspace} 
 \newcommand{\jfjgRSTAR}{\ensuremath{0.678 \pm 0.034}\xspace} 
 \newcommand{\baeiRSTAR}{\ensuremath{1.094 \pm 0.041}\xspace} 
 \newcommand{\bjieRSTAR}{\ensuremath{0.855 \pm 0.034}\xspace} 
 \newcommand{\gghbRSTAR}{\ensuremath{1.760 \pm 0.075}\xspace} 
 \newcommand{\ggacRSTAR}{\ensuremath{0.696 \pm 0.023}\xspace} 
 \newcommand{\egijRSTAR}{\ensuremath{0.879 \pm 0.034}\xspace} 
 \newcommand{\hadfRSTAR}{\ensuremath{0.956 \pm 0.037}\xspace} 
 \newcommand{\hidfRSTAR}{\ensuremath{0.840^{+0.047}_{-0.034} }\xspace} 
 \newcommand{\bebbRSTAR}{\ensuremath{0.699 \pm 0.023}\xspace} 
 \newcommand{\ecdiRSTAR}{\ensuremath{1.279 \pm 0.052}\xspace} 
 \newcommand{\gedgRSTAR}{\ensuremath{0.809 \pm 0.032}\xspace} 
 \newcommand{\jgbhRSTAR}{\ensuremath{0.638 \pm 0.020}\xspace} 
 \newcommand{\ghijRSTAR}{\ensuremath{0.876 \pm 0.036}\xspace} 
 \newcommand{\fdecRSTAR}{\ensuremath{1.060 \pm 0.042}\xspace} 
 \newcommand{\deffRSTAR}{\ensuremath{0.910 \pm 0.038}\xspace} 
 \newcommand{\hbdaRSTAR}{\ensuremath{0.721 \pm 0.025}\xspace} 
 \newcommand{\eiadRSTAR}{\ensuremath{0.995 \pm 0.042}\xspace} 
 \newcommand{\ifgjRSTAR}{\ensuremath{0.675 \pm 0.033}\xspace} 
 \newcommand{\cffcRSTAR}{\ensuremath{0.468 \pm 0.019}\xspace} 
 \newcommand{\egbeTEFF}{\ensuremath{4300^{+107}_{-100}}\xspace} 
 \newcommand{\egbeLOGG}{\ensuremath{4.566 \pm 0.036}\xspace} 
 \newcommand{\egbeFEH}{\ensuremath{0.376 \pm 0.095}\xspace} 
 \newcommand{\egbeSVAL}{---\xspace} 
 \newcommand{\egbeRPHK}{---\xspace} 
 \newcommand{\egbeVSINI}{---\xspace} 
 \newcommand{\egbeMSTAR}{\ensuremath{0.688 \pm 0.069}\xspace} 
 \newcommand{\egbeRSTAR}{\ensuremath{0.715^{+0.043}_{-0.040}}\xspace} 
 \newcommand{\hagfTEFF}{\ensuremath{3896 \pm 189}\xspace} 
 \newcommand{\hagfLOGG}{\ensuremath{4.734 \pm 0.062}\xspace} 
 \newcommand{\hagfFEH}{\ensuremath{-0.32 \pm 0.13}\xspace} 
 \newcommand{\hagfSVAL}{---\xspace} 
 \newcommand{\hagfRPHK}{---\xspace} 
 \newcommand{\hagfVSINI}{---\xspace} 
 \newcommand{\hagfMSTAR}{\ensuremath{0.601 \pm 0.089}\xspace} 
 \newcommand{\hagfRSTAR}{\ensuremath{0.561 \pm 0.068}\xspace} 
 \newcommand{\ihidTEFF}{\ensuremath{5520 \pm 60}\xspace} 
 \newcommand{\ihidLOGG}{\ensuremath{4.50 \pm 0.05}\xspace} 
 \newcommand{\ihidFEH}{\ensuremath{0.08 \pm 0.04}\xspace} 
 \newcommand{\ihidSVAL}{---\xspace} 
 \newcommand{\ihidRPHK}{\ensuremath{-4.726}\xspace} 
 \newcommand{\ihidVSINI}{\ensuremath{0.2}\xspace} 
 \newcommand{\ihidMSTAR}{\ensuremath{0.934\pm0.038}\xspace} 
 \newcommand{\ihidRSTAR}{\ensuremath{0.899^{+0.035}_{-0.033}}\xspace} 
 \newcommand{\ddigTEFF}{\ensuremath{5261 \pm 60}\xspace} 
 \newcommand{\ddigLOGG}{\ensuremath{4.47 \pm 0.05}\xspace} 
 \newcommand{\ddigFEH}{\ensuremath{0.04 \pm 0.05}\xspace} 
 \newcommand{\ddigSVAL}{---\xspace} 
 \newcommand{\ddigRPHK}{\ensuremath{-5.04}\xspace} 
 \newcommand{\ddigVSINI}{\ensuremath{1.17 \pm 1.1}\xspace} 
 \newcommand{\ddigMSTAR}{\ensuremath{0.866 \pm 0.033}\xspace} 
 \newcommand{\ddigRSTAR}{\ensuremath{0.872 \pm 0.057}\xspace} 

